TikZ-FeynHand: Basic User Guide

This is a userguide for the LaTex package Tikz-FeynHand at https://ctan.org/pkg/tikz-feynhand which let's you draw Feynman diagrams using TikZ. It contains many examples and a 5-minute introduction to TikZ. The package is a low-end modification of the package TikZ-Feynman at https://ctan.org/pkg/tikz-feynman, one of whose principal advantages is the automatic generation of diagrams, for which it needs LuaTex. FeynHand only provides the manual mode and hence runs in LaTex without any reference to LuaTex. In addition it provides some NEW STYLES for vertices and propagators, alternative SHORTER KEYWORDS in addition to TikZ-Feynman's longer ones, some shortcut commands for QUICKLY CUSTOMIZING the diagrams' look, and the new feature to put one propagator "ON TOP" of another.

==> tikzfeynhand.keys.code.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TikZ-FeynHand, Version 1.0.0 of 2018/01/31
% Feynhand Diagrams with TikZ (LaTex manual version)
% Copyright (C) 2018 Max Dohse
% Copyright (C) 2016 Joshua Ellis
%
%
% This LaTeX file and the whole package are free: 
% you can redistribute it and/or modify it under the
% terms of the GNU General Public License as published by the Free Software Foundation, 
% either version 3 of the License, or (at your option) any later version.
%
% This file is a modification of the file tikzfeynman.keys.code.tex
% of the package tikz-feynman (version 1.1.0 of 2016/02/05)
% which is available online at https://ctan.org/pkg/tikz-feynman
% for a list of changes, see the file CHANGES.TXT
%
% available at https://ctan.org/pkg/tikz-feynhand
% The Current Maintainer of this work is Max Dohse.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Lengths
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newlength{\feynhanddotsize}
\setlength{\feynhanddotsize}{1.5mm}

\newlength{\feynhandblobsize}
\setlength{\feynhandblobsize}{7.5mm}

\newlength{\feynhandlinesize}
\setlength{\feynhandlinesize}{0.5pt}

\newlength{\feynhandarrowsize}
\setlength{\feynhandarrowsize}{6pt}

\newlength{\feynhandtopsep}
\setlength{\feynhandtopsep}{18\feynhandlinesize}

%% Colors
\newcommand{\feynhandtopsepcolor}{white}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Shapes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Crossed Circle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{crossed circle}
{
  \inheritsavedanchors[from=circle]
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}

  \inheritbackgroundpath[from=circle]

  \foregroundpath{
    % Compute south west
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by-0.707107\pgf@xc
    \advance\pgf@y by-0.707107\pgf@xc
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y  % Store coordinates
    % Compute north east point
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by0.707107\pgf@xc
    \advance\pgf@y by0.707107\pgf@xc
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y  % Store coordinates
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfsetarrowsstart{}
    \pgfsetarrowsend{}
 }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Decorations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete Sines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete sines replaces the path with a whole number of sine waves.
%% Thanks to http://tex.stackexchange.com/a/134516/26980
\pgfdeclaredecoration{complete sines}{initial}
{
  %% Begin by computing the overall path length and find how many sine waves we
  %% can fit in.  Nothing happens beyond the computation.
  \state{initial}[
    width=+0pt,
    next state=move,
    persistent precomputation={
      \def\tikzfeynhand@cs@angle@step{30}
      \def\tikzfeynhand@cs@current@angle{0}
      \pgfmathsetlengthmacro{\tikzfeynhand@cs@points@per@step}{
        \pgfdecoratedinputsegmentlength
        / int(\pgfdecoratedinputsegmentlength
        / \pgfdecorationsegmentlength)
        / 360
        * \tikzfeynhand@cs@angle@step}
    },
  ]{}
  %% Move to the origin to the path
  \state{move}[
    width=+\tikzfeynhand@cs@points@per@step,
    next state=draw
  ]{
    \pgfpathmoveto{\pgfpointorigin}
  }
  %% Draw the sine wave itself.  This computes the value every 20 degrees and draws straight edges.
  \state{draw}[
    width=+\tikzfeynhand@cs@points@per@step,
    switch if less than=1.25*\tikzfeynhand@cs@points@per@step to final, % <- bit of a hack
    persistent postcomputation={
      \pgfmathparse{mod(\tikzfeynhand@cs@current@angle+\tikzfeynhand@cs@angle@step, 360)}
      \let\tikzfeynhand@cs@current@angle=\pgfmathresult%
    },
  ]{
%    \pgfmathparse{sin(\tikzfeynhand@cs@current@angle) * \pgfmetadecorationsegmentamplitude / 2}
    \pgfmathparse{sin(\tikzfeynhand@cs@current@angle) * 3 * \feynhandlinesize / 2}
    \tikz@decoratepathfalse
    \pgfpathlineto{\pgfqpoint{0pt}{\pgfmathresult pt}}%
  }

  \state{final}{
    \ifdim\pgfdecoratedremainingdistance>0pt\relax
      \pgfpathlineto{\pgfpointdecoratedpathlast}
    \fi
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Keys
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzfeynhandset{
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Hooks
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  execute at begin feynhand/.code={},
  execute at end feynhand/.code={},
  every feynhand/.style={/tikzfeynhand/every feynhand@@/.append style={#1}},
  every feynhand@@/.style={
    /tikzfeynhand/.cd,
    },
  execute at begin feynhand@@/.code={}                     %% Internal version
  execute at end feynhand@@/.code={},                      %% Internal version
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Vertices
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every vertex@@/.style={
    /tikz/shape=coordinate,
  },
  every vertex/.style={/tikzfeynhand/every vertex@@/.append style={#1}},
  vertex/.style={
    /tikzfeynhand/every vertex@@,
  },
  %% DOTS + friends
  every dot@@/.style={
    /tikz/shape=circle,
    /tikz/draw,
    /tikz/fill,
    /tikz/inner sep=0pt,
    /tikz/outer sep=0pt,
    /tikz/minimum size=\feynhanddotsize,
    /tikz/line width = \feynhandlinesize,
  },
  every dot/.style={/tikzfeynhand/every dot@@/.append style={#1}},
  dot/.style={
    /tikzfeynhand/every dot@@,
  },
  every squaredot@@/.style={
    /tikz/shape=rectangle,
  },
  every squaredot/.style={/tikzfeynhand/every squaredot@@/.append style={#1}},
  squaredot/.style={
    /tikzfeynhand/every dot@@,
    /tikzfeynhand/every squaredot@@,
  },
  every ringdot@@/.style={
    /tikz/fill=none,
  },
  every ringdot/.style={/tikzfeynhand/every ringdot@@/.append style={#1}},
  ringdot/.style={
    /tikzfeynhand/every dot@@,
    /tikzfeynhand/every ringdot@@,
  },
  every crossdot@@/.style={
    /tikz/fill=none,
    /tikz/shape=crossed circle,
    /tikz/minimum size=2\feynhanddotsize,
  },
  every crossdot/.style={/tikzfeynhand/every crossdot@@/.append style={#1}},
  crossdot/.style={
    /tikzfeynhand/every dot@@,
    /tikzfeynhand/every crossdot@@,
  },
  %% BLOBS -------------------------------------------------
    every blob@@/.style={
    /tikz/shape=circle,
    /tikz/draw,
    /tikz/fill,
    /tikz/outer sep={0.5*\the\feynhandlinesize},
    /tikz/inner sep=0pt,
    /tikz/minimum size=\feynhandblobsize,
    /tikz/line width = \feynhandlinesize,
  },
  every blob/.style={/tikzfeynhand/every blob@@/.append style={#1}},
  blob/.style={
    /tikzfeynhand/every blob@@,
    /tikz/fill=black,
  },
  every ringblob@@/.style={
  },
  every ringblob/.style={/tikzfeynhand/every ringblob@@/.append style={#1}},
  ringblob/.style={
    /tikzfeynhand/every blob@@,
    /tikzfeynhand/every ringblob@@,
    /tikz/fill=white,
  },
  every NWblob@@/.style={
  },
  every NWblob/.style={/tikzfeynhand/every NWblob@@/.append style={#1}},
  NWblob/.style={
    /tikzfeynhand/every blob@@,
    /tikzfeynhand/every NWblob@@,
    /tikz/fill=none,
    /tikz/pattern=north west lines,
  },
  every NEblob@@/.style={
  },
  every NEblob/.style={/tikzfeynhand/every NEblob@@/.append style={#1}},
  NEblob/.style={
    /tikzfeynhand/every blob@@,
    /tikzfeynhand/every NEblob@@,
    /tikz/fill=none,
    /tikz/pattern=north east lines,
  },
  every grayblob@@/.style={
  },
  every grayblob/.style={/tikzfeynhand/every grayblob@@/.append style={#1}},
  grayblob/.style={
    /tikzfeynhand/every blob@@,
    /tikzfeynhand/every grayblob@@,
    /tikz/fill=gray!50!white,
  },
  %% PARTICLES
  every particle@@/.style={
    /tikz/shape=rectangle,
    /tikz/draw=none,
    /tikz/fill=none,
    /tikz/inner sep=0.3333em,
    /tikz/outer sep={0.5*\the\feynhandlinesize},
  },
  every particle/.style={/tikzfeynhand/every particle@@/.append style={#1}},
  particle/.style args={#1}{
    /tikzfeynhand/every particle@@,
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Edge styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Arrow Style
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  arrow size/.store in=\tikzfeynhand@arrow@size,
  arrow size=\feynhandarrowsize,
  with arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          %xshift=0.5mm,
          xshift=-0.166666\feynhandarrowsize,
          fill,
          inner sep=0mm,
          minimum width = \tikzfeynhand@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  with reversed arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          %xshift=0.5mm,
          xshift=0.166666\feynhandarrowsize,
          rotate=180,
          fill,
          inner sep=0mm,
          minimum width = \tikzfeynhand@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  %% Base Edge Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every edge@@/.style={},
  every edge/.style={/tikzfeynhand/every edge@@/.append style={#1}},
  %% Specific Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every plain@@/.style={
    /tikz/draw=none,
    /tikz/line width = \feynhandlinesize,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
    },
  },
  every plain/.style={/tikzfeynhand/every plain@@/.append style={#1}},
  plain/.style={
    /tikzfeynhand/every plain@@,
  },
  every top@@/.style={
    /tikz/preaction={draw=\feynhandtopsepcolor,line width=\feynhandtopsep} 
  },
  every top/.style={/tikzfeynhand/every top@@/.append style={#1}},
  top/.style={
    /tikzfeynhand/every top@@,
  },
  every boson@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/line width = \feynhandlinesize,
      /tikz/decoration={
        complete sines,
        amplitude=3\feynhandlinesize,
        segment length=7.5\feynhandlinesize,
      },
      /tikz/decorate=true,
    },
  },
  every boson/.style={/tikzfeynhand/every boson@@/.append style={#1}},
  boson/.style={
    /tikzfeynhand/every boson@@,
  },
  every charged boson@@/.style={
    /tikzfeynhand/with arrow=0.5,
  },
  every charged boson/.style={/tikzfeynhand/every charged boson@@/.append style={#1}},
  charged boson/.style={
    /tikzfeynhand/boson,
    /tikzfeynhand/every charged boson@@,
  },
  every anti charged boson@@/.style={
    /tikzfeynhand/with reversed arrow=0.5,
  },
  every anti charged boson/.style={/tikzfeynhand/every anti charged boson@@/.append style={#1}},
  anti charged boson/.style={
    /tikzfeynhand/boson,
    /tikzfeynhand/every anti charged boson@@,
  },
  every photon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/line width = \feynhandlinesize,
      /tikz/decoration={
        complete sines,
        amplitude=3\feynhandlinesize,
        segment length=7.5\feynhandlinesize,
      },
      /tikz/decorate=true,
    },
  },
  every photon/.style={/tikzfeynhand/every photon@@/.append style={#1}},
  photon/.style={
    /tikzfeynhand/every photon@@,
  },
  every scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dashed,
      /tikz/line width = \feynhandlinesize,
    },
  },
  every scalar/.style={/tikzfeynhand/every scalar@@/.append style={#1}},
  scalar/.style={
    /tikzfeynhand/every scalar@@,
  },
  every charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynhand/with arrow=0.5,
    },
  },
  every charged scalar/.style={/tikzfeynhand/every charged scalar@@/.append style={#1}},
  charged scalar/.style={
    /tikzfeynhand/scalar,
    /tikzfeynhand/every charged scalar@@,
  },
  every anti charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynhand/with reversed arrow=0.5,
    },
  },
  every anti charged scalar/.style={/tikzfeynhand/every anti charged scalar@@/.append style={#1}},
  anti charged scalar/.style={
    /tikzfeynhand/scalar,
    /tikzfeynhand/every anti charged scalar@@,
  },
  every ghost@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dotted,
      /tikz/line width = 2\feynhandlinesize,
    },
  },
  every ghost/.style={/tikzfeynhand/every ghost@@/.append style={#1}},
  ghost/.style={
    /tikzfeynhand/every ghost@@,
  },
  every charged ghost@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynhand/with arrow=0.5,
    },
  },
  every charged ghost/.style={/tikzfeynhand/every charged ghost@@/.append style={#1}},
  charged ghost/.style={
    /tikzfeynhand/ghost,
    /tikzfeynhand/every charged ghost@@,
  },
  every anti charged ghost@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynhand/with reversed arrow=0.5,
    },
  },
  every anti charged ghost/.style={/tikzfeynhand/every anti charged ghost@@/.append style={#1}},
  anti charged ghost/.style={
    /tikzfeynhand/ghost,
    /tikzfeynhand/every anti charged scalar@@,
  },
  every fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/line width = \feynhandlinesize,
      /tikzfeynhand/with arrow=0.5,
    },
  },
  every fermion/.style={/tikzfeynhand/every fermion@@/.append style={#1}},
  fermion/.style={
    /tikzfeynhand/every fermion@@,
  },
  every anti fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/line width = \feynhandlinesize,
      /tikzfeynhand/with reversed arrow=0.5,
    },
  },
  every anti fermion/.style={/tikzfeynhand/every anti fermion@@/.append style={#1}},
  anti fermion/.style={
    /tikzfeynhand/every anti fermion@@,
  },
  every majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynhand/with arrow=0.33,
      /tikzfeynhand/with reversed arrow=0.73,
      /tikz/line width = \feynhandlinesize,
    },
  },
  every majorana/.style={/tikzfeynhand/every majorana@@/.append style={#1}},
  majorana/.style={
    /tikzfeynhand/every majorana@@,
  },
  every anti majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynhand/with reversed arrow=0.33,
      /tikzfeynhand/with arrow=0.73,
      /tikz/line width = \feynhandlinesize,
    },
  },
  every anti majorana/.style={/tikzfeynhand/every anti majorana@@/.append style={#1}},
  anti majorana/.style={
    /tikzfeynhand/every anti majorana@@,
  },
  every gluon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/line width = \feynhandlinesize,
      /tikz/decoration={
        coil,
        aspect=1.2,
        mirror,
        amplitude=3\feynhandlinesize,
        segment length=8\feynhandlinesize,
      },
      /tikz/decorate=true,
    },
  },
  every gluon/.style={/tikzfeynhand/every gluon@@/.append style={#1}},
  gluon/.style={
    /tikzfeynhand/every gluon@@,
  },
  % short versions of style names
  pho/.style={
    /tikzfeynhand/photon,
  },
  bos/.style={
    /tikzfeynhand/boson,
  },
  antbos/.style={
    /tikzfeynhand/anti charged boson,
  },
  chabos/.style={
    /tikzfeynhand/charged boson,
  },
  sca/.style={
  	/tikzfeynhand/scalar,
  },
  chasca/.style={
  	/tikzfeynhand/charged scalar,
  },
  antsca/.style={
    /tikzfeynhand/anti charged scalar,
  },
  fer/.style={
    /tikzfeynhand/fermion,
  },
  antfer/.style={
    /tikzfeynhand/anti fermion,
  },
  gho/.style={
    /tikzfeynhand/ghost,
  },
  chagho/.style={
    /tikzfeynhand/charged ghost,
  },
  antgho/.style={
    /tikzfeynhand/anti charged ghost,
  },
  glu/.style={
    /tikzfeynhand/gluon,
  },
  maj/.style={
    /tikzfeynhand/majorana,
  },
  antmaj/.style={
    /tikzfeynhand/anti majorana,
  },
  %% Insertions
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  insertion/.search also={/tikzfeynhand,/tikz},
  %% Parameters
  insertion/size/.store in=\tikzfeynhand@insertion@size,
  insertion/size=5\feynhandlinesize,
  insertion/style/.store in=\tikzfeynhand@insertion@style,
  insertion/style={},
  %% Styles
  insertion@@/.style args={[#1]#2}{
    /tikz/line width = \feynhandlinesize,
    /tikz/decoration={
      markings,
      mark=at position #2 with {
        \tikzfeynhandset{insertion/.cd,#1}
        \draw [\tikzfeynhand@insertion@style] (-\tikzfeynhand@insertion@size, -\tikzfeynhand@insertion@size) -- (\tikzfeynhand@insertion@size, \tikzfeynhand@insertion@size);
        \draw [\tikzfeynhand@insertion@style] (-\tikzfeynhand@insertion@size, \tikzfeynhand@insertion@size) -- (\tikzfeynhand@insertion@size, -\tikzfeynhand@insertion@size);
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  insertion@@/.default={[]0.5},
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Momentum arrows
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  momentum/.search also={/tikzfeynhand,/tikz},
  %% Parameters
  momentum/label distance/.store in=\tikzfeynhand@momentum@label@distance,
  momentum/label distance=0pt,
  momentum/arrow distance/.store in=\tikzfeynhand@momentum@arrow@distance,
  momentum/arrow distance={\the\feynhandarrowsize},
  momentum/arrow shorten/.store in=\tikzfeynhand@momentum@arrow@shorten,
  momentum/arrow shorten=0.2,
  momentum/label style/.store in=\tikzfeynhand@momentum@label@style,
  momentum/label style={},
  momentum/arrow style/.store in=\tikzfeynhand@momentum@arrow@style,
  momentum/arrow style={},
  momentum/arrow thickness/.store in=\tikzfeynhand@momentum@arrow@thickness,
  momentum/arrow thickness={0.64*\the\feynhandlinesize},
  momentum/arrow size/.store in=\tikzfeynhand@momentum@arrow@size,
  momentum/arrow size={0.8*\the\feynhandarrowsize},
  %% Styles
  momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynhand@momentum@arrow@shorten + (1-2 * \tikzfeynhand@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynhand@momentum@arrow@shorten + (1-2 * \tikzfeynhand@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynhand@momentum@arrow@shorten + (1-2 * \tikzfeynhand@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynhand@momentum@arrow@shorten + (1-2 * \tikzfeynhand@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynhandset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynhand@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynhand@momentum@arrow@shorten] (tf@m@2);
          \draw [-{Stealth[length=\tikzfeynhand@momentum@arrow@size]},
          		line width=\tikzfeynhand@momentum@arrow@thickness, 
          		\tikzfeynhand@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynhand@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynhand@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynhand@momentum@label@distance,
                      \tikzfeynhand@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Modifiers
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  half left/.style={
    /tikz/bend left=90,
  },
  half right/.style={
    /tikz/bend right=90,
  },
  quarter left/.style={
    /tikz/bend left=45,
  },
  quarter right/.style={
    /tikz/bend right=45,
  },
}

\endinput

==> tikzlibraryfeynhand.code.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TikZ-FeynHand, Version 1.0.0 of 2018/01/31
% Feynhand Diagrams with TikZ (LaTex manual version)
% Copyright (C) 2018 Max Dohse
% Copyright (C) 2016 Joshua Ellis
%
% This LaTeX file and the whole package are free: 
% you can redistribute it and/or modify it under the
% terms of the GNU General Public License as published by the Free Software Foundation, 
% either version 3 of the License, or (at your option) any later version.
%
% This file is a modification of the file tikzlibraryfeynman.code.tex
% of the package tikz-feynman (version 1.1.0 of 2016/02/05)
% which is available online at https://ctan.org/pkg/tikz-feynman
% for a list of changes, see the file CHANGES.TXT
%
% available at https://ctan.org/pkg/tikz-feynhand
% The Current Maintainer of this work is Max Dohse.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Pre-requisites
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usetikzlibrary{
  arrows.meta,
  calc,
  decorations,
  decorations.markings,
  decorations.pathmorphing,
  decorations.pathreplacing,
  external,
  patterns,
  positioning,
  shapes.geometric,
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Function definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Miscellaneous functions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynhand@empty{}

%% Key Manager
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Setup the tikz-feynhand key family
\pgfkeys{
  /tikzfeynhand/.is family,
  /tikzfeynhand/.search also={/tikz},
}

%% |\tikzfeynhandset| allows keys that belong with tikz-feynhand to be easily set.
\def\tikzfeynhandset{\pgfqkeys{/tikzfeynhand}}

%% Version check
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Check which version is expected and which is installed
\def\tikzfeynhand@compat@parse#1.#2.#3\pgfeov{
  \edef\tikzfeynhand@compat@major{#1}
  \edef\tikzfeynhand@compat@minor{#2}
  \edef\tikzfeynhand@compat@patch{#3}
  \edef\tikzfeynhand@compat{#1.#2.#3}
}
\let\tikzfeynhand@compat=\tikzfeynhand@empty
\pgfkeyslet{/tikzfeynhand/compat/.@cmd}{\tikzfeynhand@compat@parse}
\ProcessPgfPackageOptions{/tikzfeynhand}

\AtBeginDocument{
  \ifx\tikzfeynhand@version\tikzfeynhand@compat\else
    \ifx\tikzfeynhand@compat\tikzfeynhand@empty
      \PackageWarning{tikz-feynhand}{Consider loading TikZ-Feynhand with \string\usepackage[compat=\tikzfeynhand@version]{tikz-feynhand} so that you can be warned if TikZ-Feynhand changes.}
    \else
      \ifx\tikzfeynhand@compat@major\tikzfeynhand@version@major
        \ifx\tikzfeynhand@compat@minor\tikzfeynhand@version@minor
          \ifx\tikzfeynhand@compat@patch\tikzfeynhand@version@patch\else
            \PackageInfo{tikz-feynhand}{The preamble requested version \tikzfeynhand@compat, but the system version is \tikzfeynhand@version.  This should cause no issue.}
          \fi
        \else
          \PackageWarning{tikz-feynhand}{The preamble requested version \tikzfeynhand@compat, but the system version is \tikzfeynhand@version.  This may change some diagrams.}
        \fi
      \else
        \PackageError{tikz-feynhand}{The preamble requested version \tikzfeynhand@compat, but the system version is \tikzfeynhand@version.  They are most likely incompatible.  Please download the appropriate version from jpellis.me/projects/tikz-feynhand.}
      \fi
    \fi
  \fi
}

%% Feynhand Environment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Provide `\begin{feynhand} ... \end{feynhand}` within TikZ pictures.
\tikzaddtikzonlycommandshortcutlet\feynhand\tikzfeynhand@environment@feynhand
\tikzaddtikzonlycommandshortcutlet\endfeynhand\endtikzfeynhand@environment@feynhand

%% \begin{feynhand}...\end{feynhand}
\def\tikzfeynhand@environment@feynhand{%
  \pgfutil@ifnextchar[{\tikzfeynhand@environment@feynhand@opt}
  {\tikzfeynhand@environment@feynhand@opt[]}}

\def\tikzfeynhand@environment@feynhand@opt[#1]{%
  \begingroup
  %% Local overrides
  \let\tikz@@scan@fig=\tikzfeynhand@scan@fig
  %% Local commands
  \let\vertex=\tikzfeynhand@commands@vertex
  \let\propagator=\tikzfeynhand@commands@propagator
  \let\propag=\propagator
  %% Opening hooks
  \scope
  \tikzfeynhand@tikz@search@tikzfeynhand
  \pgfkeys{/tikzfeynhand/every feynhand@@,#1}
  \pgfkeysvalueof{/tikzfeynhand/execute at begin feynhand@@}%
  \pgfkeysvalueof{/tikzfeynhand/execute at begin feynhand}%
  }

\def\endtikzfeynhand@environment@feynhand{%	
  %% Closing hooks
  \pgfkeysvalueof{/tikzfeynhand/execute at end feynhand}%
  \pgfkeysvalueof{/tikzfeynhand/execute at end feynhand@@}%
  \endscope
  \endgroup
  }

%%% Allow empty nodes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\iftikzfeynhandallowemptynode
\newif\iftikzfeynhandvertex
\def\tikzfeynhand@scan@fig{%
  \pgfutil@ifnextchar a{\tikz@fig@scan@at}
    {\pgfutil@ifnextchar({\tikz@fig@scan@name}
      {\pgfutil@ifnextchar[{\tikz@fig@scan@options}%
        {\pgfutil@ifnextchar\bgroup{\tikz@fig@main}%
          {\iftikzfeynhandvertex%
             \tikzset{/tikzfeynhand/every vertex@@}%
             \iftikzfeynhandallowemptynode%
               \else%
               \tikzset{/tikzfeynhand/particle}%
               \fi%
            \fi%
            \tikz@fig@main{}
          }
        }
      }
    }
}

%% Include /tikzfeynhand in the search path
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynhand@tikz@search@tikzfeynhand{%
  \pgfkeys{/tikz/.unknown/.code=%
    \let\tikz@key\pgfkeyscurrentname%
    %% Is it a tikzfeynhand key?
    \pgfkeys{/tikzfeynhand/\tikz@key/.try={##1}}%
    \ifpgfkeyssuccess%
    \else%
      %% Is it a pgf key?
      \pgfkeys{/pgf/\tikz@key/.try={##1}}%
      \ifpgfkeyssuccess%
      \else%
        \expandafter\pgfutil@in@\expandafter!\expandafter{\tikz@key}%
        \ifpgfutil@in@%
          %% this is a color!
          \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
          \edef\tikz@textcolor{\tikz@key}%
        \else%
          \pgfutil@doifcolorelse{\tikz@key}
          {%
            \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
            \edef\tikz@textcolor{\tikz@key}%
          }%
          {%
            %% Ok, second chance: This might be an arrow specification:
            \expandafter\pgfutil@in@\expandafter-\expandafter{\tikz@key}%
            \ifpgfutil@in@%
              %% Ah, an arrow spec!
              \expandafter\tikz@processarrows\expandafter{\tikz@key}%
            \else%
              %% Ok, third chance: A shape!
              \expandafter\ifx\csname pgf@sh@s@\tikz@key\endcsname\relax%
                \pgfkeys{/errors/unknown key/.expand
                once=\expandafter{\expandafter/\expandafter t\expandafter
                i\expandafter k\expandafter z\expandafter/\tikz@key}{##1}}%
              \else%
                \edef\tikz@shape{\tikz@key}%
              \fi%
            \fi%
          }%
        \fi%
      \fi%
    \fi%
  }
}


%% Vertex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% SEE ALSO \vertex above!
%% Adapted from |\coordinate| code
\def\tikzfeynhand@commands@vertex{%
  \path \pgfextra{\tikzfeynhandallowemptynodetrue}
        \pgfextra{\tikzfeynhandvertextrue}
        node}

%% Propagators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\tikzfeynhand@commands@propagator}[1][]{\draw [#1]}

%% Optional argument in style key
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynhand@key@opt#1[#2]#3\pgfeov{%
  \tikzfeynhandset{#1={[#2]#3}}}

%% Insertion
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynhand@insertion{%
  \pgfutil@ifnextchar[{\tikzfeynhand@key@opt{insertion@@}}
  {\tikzfeynhand@key@opt{insertion@@}[]}}
\pgfkeyslet{/tikzfeynhand/insertion/.@cmd}{\tikzfeynhand@insertion}

%% Momentum
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynhand@momentum@std{%
  \pgfutil@ifnextchar[{\tikzfeynhand@key@opt{momentum@@}}
  {\tikzfeynhand@key@opt{momentum@@}[]}}
\pgfkeyslet{/tikzfeynhand/momentum/.@cmd}{\tikzfeynhand@momentum@std}

\def\tikzfeynhand@momentum@stdp{%
  \pgfutil@ifnextchar[{\tikzfeynhand@key@opt{momentum'@@}}
  {\tikzfeynhand@key@opt{momentum'@@}[]}}
\pgfkeyslet{/tikzfeynhand/momentum'/.@cmd}{\tikzfeynhand@momentum@stdp}

\def\tikzfeynhand@momentum@stdr{%
  \pgfutil@ifnextchar[{\tikzfeynhand@key@opt{reversed momentum@@}}
  {\tikzfeynhand@key@opt{reversed momentum@@}[]}}
\pgfkeyslet{/tikzfeynhand/reversed momentum/.@cmd}{\tikzfeynhand@momentum@stdr}

\def\tikzfeynhand@momentum@stdrp{%
  \pgfutil@ifnextchar[{\tikzfeynhand@key@opt{reversed momentum'@@}}
  {\tikzfeynhand@key@opt{reversed momentum'@@}[]}}
\pgfkeyslet{/tikzfeynhand/reversed momentum'/.@cmd}{\tikzfeynhand@momentum@stdrp}

% short versions of momentum styles
\pgfkeyslet{/tikzfeynhand/rmomentum/.@cmd}{\tikzfeynhand@momentum@stdr}
\pgfkeyslet{/tikzfeynhand/rmomentum'/.@cmd}{\tikzfeynhand@momentum@stdrp}

\pgfkeyslet{/tikzfeynhand/mom/.@cmd}{\tikzfeynhand@momentum@std}
\pgfkeyslet{/tikzfeynhand/mom'/.@cmd}{\tikzfeynhand@momentum@stdp}

\pgfkeyslet{/tikzfeynhand/revmom/.@cmd}{\tikzfeynhand@momentum@stdr}
\pgfkeyslet{/tikzfeynhand/revmom'/.@cmd}{\tikzfeynhand@momentum@stdrp}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input tikzfeynhand.keys.code.tex

\endinput
